API Misuse Detection An Immune System inspired Approach

APIs are essential ingredients for developing complex software systems. However, they are difficult to learn and to use. Thus, developers may misuse them, which results in various types of issues. In this paper, we explore the use of a bio-inspired approach (artificial immune system) to detect API misuses in client code. We built APIMMUNE, a novel API misuse detector. We collect normal usages of a given APIs from the set of client programs using the APIs, especially after some API usages were fixed in those programs. The normal API usages are considered as normal body cells. We transform them into normal-usage signatures. Then, artificial detectors are randomly generated by generating artificial deviations from these usages with the objective of being different from the normal usage signatures. The generated detectors have the ability to detect risky uses of APIs exactly as the immune system detects foreign cells of the organism. Moreover, for the detection purpose, only the artificial detectors are necessary, without the need to disclose the code used to generate them. Our approach was evaluated on the misuses dataset of three APIs as well as on known misuses from a state of the art APIs misuses benchmarking dataset. APIMMUNE was also compared to four state-of-the-art API misuse detection tools. The results show that APIMMUNE has good detection accuracy and performance, and it can complement pattern-based tools for uncommon misuses detection.

==> ais.tex <==
\section{BIS-based detection of API misuses}
\label{sec:detection_algorithm}

In this section, we discuss the formulation and rational behind the
choice of the biological immune-system as an inspiration to develop
{\tool}. We present the principles of the artificial immune system
algorithm (AIS), a simplified abstraction of the BIS, and the
adaptation of this to the API-misuse detection problem.


\subsection{Running Example}
An API misuse is a specific issue which results from the violation of
the API specifications. It is an unexpected utilization of the APIs. For
example, in Figure~\ref{Example}, the resource \textit{BufferedReader}
is initialized (line 2), used to read each line (line 4) but not
closed at the end. It is a classic example of \textit{BufferedReader}
misuse. This misuse is an instance of one of the 13 types of common
misuses, identified by the authors of the benchmark \emph{MuBench} in
\cite{MuBench}, i.e., missing call.
%
In this misuse, if the resource is not closed, it means that no other
processes can access it. This misuse can cause exceptions and
perhaps corrupt the resources. Thus, we need to detect this risk early.


\begin{figure}
\includegraphics[width=3in]{fig/testGroum_java}
\caption{\textit{BufferedReader} Misuse Example}
\label{Example}
\end{figure}

In this work, we formulate an API usage as follows.

\begin{Definition}[API Usage]
An API usage is a fragment of code that involves the API classes and
methods in certain libraries.
\end{Definition}

As an example, the code in Figure~\ref{Example} is an API usage
containing several APIs in JDK library, such as the classes
\code{StringBuffer}, \code{BufferredReader}, \code{FileReader}, etc.,
and the method calls \code{BufferedReader.readLine()},
\code{StringBuffer.append(...)}, \code{StringBuffer.length()}, etc.

We adopt GROUM, a graph-based representation for the API
usages~\cite{Grouminer}. For 

\subsection{Artificial Immune System Detection}


To protect the organism from potential pathogens, the immune system
follows a 3-steps cycle: (1) discovery, (2) identification and (3)
elimination. The discovery step detects potential pathogenes, such as
viruses and bacteria. When such an element is detected, the
identification step is responsible for checking if the identified
element is known (immune memory). Finally, in the elimination step,
the adequate response is selected depending on the identification
step. As we are concerned with the detection of API misuses, we focus
only on the discovery step and its abstraction by the AIS.

One of the most important notions in an AIS is the self. It defines
the boundaries of what is normal, and then, non-risky. For a human
being, for example, the self is defined by all the normal cells of the
body.

In the context of the API misuse detection, the selfs for APIs are the
API usages in client programs after the API usages are fixed.

In the context of the API misuse problem, the self for an API can be
defined by a set of client programs that correctly used the API in the
past. The advantage of this definition is that the self for an API
evolves as new clients correctly using the API can be added.

A second important notion in an AIS is the maturation of T-cells that
can be used to detect non-self elements. The T-cells are created
randomly and exposed to normal cells. If a T-cell matches a normal
cell, it is removed from the repertoire of immune cells to avoid the
body attacking itself. This is called negative selection. For
computation reasons, it is not possible to create a large number of
T-cells. Hence, it is important to ensure a maximum coverage while
keeping minimal the number of T-cells.

When transposing the principle of the negative selection to the
detection of API misuses, the random generation of detectors can be
implemented by a multi-objective optimization process. Indeed, if we
fix the number of detectors, the goal is to find the set of detectors
that are as much as possible different from the normal use situations
in the selected clients, but also as much as possible different
between them.

The next important notion of an AIS is the affinity computation
between a detector and an encountered cell. The affinity is a
similarity function that allows to assess if the encountered cell
belongs to self or not.

For the misuse detection, we are interested in the method level. The
goal then is to define an abstract representation of a method that
indicates how this method uses the targeted API. Such an abstraction
should ignore elements not related to the API.



==> evaluation.tex <==
\section{Preliminary evaluation}
\label{sec:evaluation}

\input{data}

\subsection{Results}
To conduct the experiments, we created 10 folds having, each, 183 cases of good uses and their equivalent
183 misuse cases. Then for each fold, we generate the detectors using the good
uses in the nine other folds. The detectors are then applied to each good or bad
use case in the fold (386=183+183) to calculate their risk scores (c.f., Section~\ref{sec:detection}).
The cases are then sorted by their scores. This allows to compute the precision and recall for each fold at k
(k cases with the highest risk scores).



Figure~\ref{fig:precision_recall} shows the distribution of the precision and recall at-250 for the ten folds.
With an average precision of 63,67\% (and a maximum of 72.5\%), our approach produces results better than a random guess (50\% for a balanced
testing sample). The average recall is also high with an average of 87,32\% (maximum of 99,45\%).



To show how the precision and recall evolve as the risk score decreases, we selected a representative fold (Figure~\ref{fig:fold7}.

\begin{table}[htp]
	\centering
	\begin{tabular}{|>{\raggedright}m{2cm}|*{6}{m{0.25in}|}}
		\hline
		\multirow{4}{*}{}&\multicolumn{3}{c|}{Max} & \multicolumn{3}{c|}{Noisy or} \\
		\cline{2-7}
		 & Iterator & http & crypto & Iterator & http & crypto \\
		\hline
		Mean score good usages & 0.2808 & 0.1505 &	0.2104	& 0.9246	& 0.4127	& 0.3763 \\
		\hline
		Mean score bad usages & 0.2865	& 0.984	& 0.1947	& 0.9483	& 0.5583	& 0.3841	\\
		\hline
		Mean precision 10\% data (\%)	& 53.78	& \textbf{70.0}	& 50.,0	& 52.70	& \textbf{66.67}	& 45.0	\\
		\hline
		Mean precision 30\% data (\%)	& 50.18	& 58.89	& 57.14	& 54.74	& \textbf{66.67} & 54.29 \\
		\hline
	\end{tabular}
	\caption{Generation process without clustering results}
  \label{tab:process0}
\end{table}

\begin{table}[htpb]
	\centering
		\begin{tabular}{|*{5}{c|}}
			\hline
			\multirow{3}{*}{}&\multicolumn{2}{c|}{Max} & \multicolumn{2}{c|}{Noisy or} \\
			\cline{2-5}
			& http & crypto & http & crypto \\
			\hline
			Mean score good usages & 0.1866 & 0.1841 & 0.4653 & 0.4227 \\
			\hline
			Mean score bad usages & 0.2286 & 0.1520 & 0.6312 & 0.3830 \\
			\hline
			Mean precision 10\% data (\%) & 53.33 & 40.0 & \textbf{60.0} & 40.0 \\
			\hline
			Mean precision 30\% data (\%) & 57.78 & 48.57 & 57.78 & 51.43 \\
			\hline
		\end{tabular}
		\caption{Generation process with clustering, and merging after evolution results}
		\label{tab:process4}
\end{table}

\begin{table}[htpb]
	\centering
		\begin{tabular}{|*{5}{c|}}
			\hline
			\multirow{3}{*}{}&\multicolumn{2}{c|}{Max} & \multicolumn{2}{c|}{Noisy or} \\
			\cline{2-5}
			& http & crypto & http & crypto \\
			\hline
			Mean score good usages & 0.1641 & 0.2064 & 0.4515 & 0.4654 \\
			\hline
			Mean score bad usages & 0.1947 & 0.2129 & 0.5303 & 0.5754 \\
			\hline
			Mean precision 10\% data (\%) & 46.67 & 45.0 & \textbf{70.0} & 55.0 \\
			\hline
			Mean precision 30\% data(\%) & 56.67 & 52.86 & 57.78 & 58.57 \\
			\hline
		\end{tabular}
		\caption{Generation process with clustering, and merging before evolution results}
		\label{tab:process5}
\end{table}

\begin{figure}
\includegraphics[width=3.25in]{fig/MUBenchCrypto.png}
\caption{Precision - Recall for javax.crypto clients on MUBench}
\label{fig:MUBenchCrypto}
\end{figure}

\begin{figure}
\includegraphics[width=3.25in]{fig/MUBenchIterator}
\caption{Precision - Recall for java.util.Iterator clients on MUBench}
\label{fig:MUBenchIterator}
\end{figure}

